On Linear Information Systems

Scott's information systems provide a categorically equivalent, intensional description of Scott domains and continuous functions. Following a well established pattern in denotational semantics, we define a linear version of information systems, providing a model of intuitionistic linear logic (a new-Seely category), with a "set-theoretic" interpretation of exponentials that recovers Scott continuous functions via the co-Kleisli construction. From a domain theoretic point of view, linear information systems are equivalent to prime algebraic Scott domains, which in turn generalize prime algebraic lattices, already known to provide a model of classical linear logic.

==> eptcsdata.tex <==
\providecommand{\event}{M. Florido and I. Mackie (Eds.): First International\\
Workshop on Linearity (LINEARITY 2009)}
\providecommand{\volume}{22}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{38}
\providecommand{\eid}{4}

